Adjusting for Confounders with Text: Challenges and an Empirical Evaluation Framework for Causal Inference

Causal inference studies using textual social media data can provide actionable insights on human behavior. Making accurate causal inferences with text requires controlling for confounding which could otherwise impart bias. Recently, many different methods for adjusting for confounders have been proposed, and we show that these existing methods disagree with one another on two datasets inspired by previous social media studies. Evaluating causal methods is challenging, as ground truth counterfactuals are almost never available. Presently, no empirical evaluation framework for causal methods using text exists, and as such, practitioners must select their methods without guidance. We contribute the first such framework, which consists of five tasks drawn from real world studies. Our framework enables the evaluation of any casual inference method using text. Across 648 experiments and two datasets, we evaluate every commonly used causal inference method and identify their strengths and weaknesses to inform social media researchers seeking to use such methods, and guide future improvements. We make all tasks, data, and models public to inform applications and encourage additional research.

==> bibliography_uncompressed.tex <==
@article{Yu2020ABO,
  title={A Bibliometric Overview of Twitter-Related Studies Indexed in Web of Science},
  author={J. Yu and Juan Mu{\~n}oz-Justicia},
  journal={Future Internet},
  year={2020},
  volume={12},
  pages={91}
}


@misc{chen2020causal,
      title={Causal Knowledge Extraction from Scholarly Papers in Social Sciences}, 
      author={Victor Zitian Chen and Felipe Montano-Campos and Wlodek Zadrozny},
      year={2020},
      eprint={2006.08904},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}



@inproceedings{joulin-etal-2017-bag,
    title = "Bag of Tricks for Efficient Text Classification",
    author = "Joulin, Armand  and
      Grave, Edouard  and
      Bojanowski, Piotr  and
      Mikolov, Tomas",
    booktitle = "Proceedings of the 15th Conference of the {E}uropean Chapter of the Association for Computational Linguistics: Volume 2, Short Papers",
    month = apr,
    year = "2017",
    address = "Valencia, Spain",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/E17-2068",
    pages = "427--431",
    abstract = "This paper explores a simple and efficient baseline for text classification. Our experiments show that our fast text classifier fastText is often on par with deep learning classifiers in terms of accuracy, and many orders of magnitude faster for training and evaluation. We can train fastText on more than one billion words in less than ten minutes using a standard multicore CPU, and classify half a million sentences among 312K classes in less than a minute.",
}



@inproceedings{lin2019universal, title = {Universal Causal Evaluation Engine: An API for empirically evaluating causal inference models}, author = {Lin, Alexander and Merchant, Amil and Sarkar, Suproteem K. and D'Amour, Alexander}, booktitle = {Proceedings of Machine Learning Research}, pages = {50--58}, year = {2019}, editor = {Thuc Duy Le and Jiuyong Li and Kun Zhang and Emre Kıcıman Peng Cui and Aapo Hyvärinen}, volume = {104}, series = {Proceedings of Machine Learning Research}, address = {Anchorage, Alaska, USA}, month = {05 Aug}, publisher = {PMLR}, pdf = {http://proceedings.mlr.press/v104/lin19a/lin19a.pdf}, url = {http://proceedings.mlr.press/v104/lin19a.html}, abstract = {A major driver in the success of predictive machine learning has been the “common task framework,” where community-wide benchmarks are shared for evaluating new algorithms. This pattern, however, is difficult to implement for causal learning tasks because the ground truth in these tasks is in general unobservable. Instead, causal inference methods are often evaluated on synthetic or semi-synthetic datasets that incorporate idiosyncratic assump- tions about the underlying data-generating process. These evaluations are often proposed in conjunction with new causal inference methods—as a result, many methods are eval- uated on incomparable benchmarks. To address this issue, we establish an API for gen- eralized causal inference model assessment, with the goal of developing a platform that lets researchers deploy and evaluate new model classes in instances where treatments are explicitly known. The API uses a common interface for each of its components, and it allows for new methods and datasets to be evaluated and saved for future benchmarking.} }

@inproceedings{Wang_Culotta_2019,
    title={When Do Words Matter? Understanding the Impact of Lexical Choice on Audience Perception Using Individual Treatment Effect Estimation},
    url={https://ojs.aaai.org/index.php/AAAI/article/view/4708},
    booktitle={AAAI},
    author={Wang, Zhao and Culotta, Aron},
    year={2019},
}


@inproceedings{choudhury2014self_disclosure,
  title={Mental Health Discourse on reddit: Self-Disclosure, Social Support, and Anonymity},
  author={Munmun De Choudhury and Sushovan De},
  booktitle={ICWSM},
  year={2014}
}


@inbook{hirano2004continuous,
author = {Hirano, Keisuke and Imbens, Guido W.},
publisher = {John Wiley & Sons, Ltd},
isbn = {9780470090459},
title = {The Propensity Score with Continuous Treatments},
booktitle = {Applied Bayesian Modeling and Causal Inference from Incomplete‐Data Perspectives},
chapter = {7},
pages = {73-84},
doi = {https://doi.org/10.1002/0470090456.ch7},
url = {https://onlinelibrary.wiley.com/doi/abs/10.1002/0470090456.ch7},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.1002/0470090456.ch7},
year = {2004},
keywords = {generalized propensity score (GPS), binary treatment case, propensity score methodology, conventional regression estimates, weak unconfoundedness, marginal structural model (MSM), asymptotic standard errors, dose-response function},
abstract = {Summary This chapter contains sections titled: Introduction The basic framework Bias removal using the GPS Estimation and inference Application: the Imbens–Rubin–Sacerdote lottery sample Conclusion}
}


@paper{landeiro2016robust,
	author = {Virgile Landeiro and Aron Culotta},
	title = {Robust Text Classification in the Presence of Confounding Bias},
	conference = {AAAI Conference on Artificial Intelligence},
	year = {2016},
	keywords = {social media; text classification; causal inference},
	abstract = {As text classifiers become increasingly used in real-time applications, it is critical to consider not only their accuracy but also their robustness to changes in the data distribution. In this paper, we consider the case where there is a confounding variable Z that influences both the text features X and the class variable Y. For example, a classifier trained to predict the health status of a user based on their online communications may be confounded by socioeconomic variables. When the influence of Z changes from training to testing data, we find that classifier accuracy can degrade rapidly. Our approach, based on Pearl's back-door adjustment, estimates the underlying effect of a text variable on the class variable while controlling for the confounding variable. Although our goal is prediction, not causal inference, we find that such adjustments are essential to building text classifiers that are robust to confounding variables. On three diverse text classifications tasks, we find that covariate adjustment results in higher accuracy than competing baselines over a range of confounding relationships (e.g., in one setting, accuracy improves from 60\% to 81\%).},

	url = {https://www.aaai.org/ocs/index.php/AAAI/AAAI16/paper/view/12445}
}

@inproceedings{pryzant2018deconfounded,
    title = "Deconfounded Lexicon Induction for Interpretable Social Science",
    author = "Pryzant, Reid  and
      Shen, Kelly  and
      Jurafsky, Dan  and
      Wagner, Stefan",
    booktitle = "Proceedings of the 2018 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long Papers)",
    month = jun,
    year = "2018",
    address = "New Orleans, Louisiana",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/N18-1146",
    doi = "10.18653/v1/N18-1146",
    pages = "1615--1625",
    abstract = "NLP algorithms are increasingly used in computational social science to take linguistic observations and predict outcomes like human preferences or actions. Making these social models transparent and interpretable often requires identifying features in the input that predict outcomes while also controlling for potential confounds. We formalize this need as a new task: inducing a lexicon that is predictive of a set of target variables yet uncorrelated to a set of confounding variables. We introduce two deep learning algorithms for the task. The first uses a bifurcated architecture to separate the explanatory power of the text and confounds. The second uses an adversarial discriminator to force confound-invariant text encodings. Both elicit lexicons from learned weights and attentional scores. We use them to induce lexicons that are predictive of timely responses to consumer complaints (controlling for product), enrollment from course descriptions (controlling for subject), and sales from product descriptions (controlling for seller). In each domain our algorithms pick words that are associated with \textit{narrative persuasion}; more predictive and less confound-related than those of standard feature weighting and lexicon induction techniques like regression and log odds.",
}


@article{schuler2017tmle,
  title={Targeted Maximum Likelihood Estimation for Causal Inference in Observational Studies},
  author={M. Schuler and Sherri Rose},
  journal={American Journal of Epidemiology},
  year={2017},
  volume={185},
  pages={65–73}
}

@article{kang2007demystifying,
author = "Kang, Joseph D. Y. and Schafer, Joseph L.",
doi = "10.1214/07-STS227",
fjournal = "Statistical Science",
journal = "Statist. Sci.",
month = "11",
number = "4",
pages = "523--539",
publisher = "The Institute of Mathematical Statistics",
title = "Demystifying Double Robustness: A Comparison of Alternative Strategies for Estimating a Population Mean from Incomplete Data",
url = "https://doi.org/10.1214/07-STS227",
volume = "22",
year = "2007"
}


@article{medvedev2019anatomy,
   title={The Anatomy of Reddit: An Overview of Academic Research},
   ISBN={9783030146832},
   ISSN={2213-8692},
   url={http://dx.doi.org/10.1007/978-3-030-14683-2_9},
   DOI={10.1007/978-3-030-14683-2_9},
   journal={Springer Proceedings in Complexity},
   publisher={Springer International Publishing},
   author={Medvedev, Alexey N. and Lambiotte, Renaud and Delvenne, Jean-Charles},
   year={2019},
   pages={183–204}
}



@article{chandrasekharan2018internet,
author = {Chandrasekharan, Eshwar and Samory, Mattia and Jhaver, Shagun and Charvat, Hunter and Bruckman, Amy and Lampe, Cliff and Eisenstein, Jacob and Gilbert, Eric},
title = {The Internet’s Hidden Rules: An Empirical Study of Reddit Norm Violations at Micro, Meso, and Macro Scales},
year = {2018},
issue_date = {November 2018},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {2},
number = {CSCW},
url = {https://doi.org/10.1145/3274301},
doi = {10.1145/3274301},
journal = {Proc. ACM Hum.-Comput. Interact.},
month = nov,
articleno = {32},
numpages = {25},
keywords = {community norms, moderation, online communities, mixed methods.}
}
  


@article{crump2009dealing,
    author = {Crump, Richard K. and Hotz, V. Joseph and Imbens, Guido W. and Mitnik, Oscar A.},
    title = "{Dealing with limited overlap in estimation of average treatment effects}",
    journal = {Biometrika},
    volume = {96},
    number = {1},
    pages = {187-199},
    year = {2009},
    month = {01},
    abstract = "{Estimation of average treatment effects under unconfounded or ignorable treatment assignment is often hampered by lack of overlap in the covariate distributions between treatment groups. This lack of overlap can lead to imprecise estimates, and can make commonly used estimators sensitive to the choice of specification. In such cases researchers have often used ad hoc methods for trimming the sample. We develop a systematic approach to addressing lack of overlap. We characterize optimal subsamples for which the average treatment effect can be estimated most precisely. Under some conditions, the optimal selection rules depend solely on the propensity score. For a wide range of distributions, a good approximation to the optimal rule is provided by the simple rule of thumb to discard all units with estimated propensity scores outside the range [0.1,0.9].}",
    issn = {0006-3444},
    doi = {10.1093/biomet/asn055},
    url = {https://doi.org/10.1093/biomet/asn055},
    eprint = {https://academic.oup.com/biomet/article-pdf/96/1/187/642537/asn055.pdf},
}




@article{lee2011weight,
    author = {Lee, Brian K. AND Lessler, Justin AND Stuart, Elizabeth A.},
    journal = {PLOS ONE},
    publisher = {Public Library of Science},
    title = {Weight Trimming and Propensity Score Weighting},
    year = {2011},
    month = {03},
    volume = {6},
    url = {https://doi.org/10.1371/journal.pone.0018174},
    pages = {1-6},
    abstract = {Propensity score weighting is sensitive to model misspecification and outlying weights that can unduly influence results. The authors investigated whether trimming large weights downward can improve the performance of propensity score weighting and whether the benefits of trimming differ by propensity score estimation method. In a simulation study, the authors examined the performance of weight trimming following logistic regression, classification and regression trees (CART), boosted CART, and random forests to estimate propensity score weights. Results indicate that although misspecified logistic regression propensity score models yield increased bias and standard errors, weight trimming following logistic regression can improve the accuracy and precision of final parameter estimates. In contrast, weight trimming did not improve the performance of boosted CART and random forests. The performance of boosted CART and random forests without weight trimming was similar to the best performance obtainable by weight trimmed logistic regression estimated propensity scores. While trimming may be used to optimize propensity score weights estimated using logistic regression, the optimal level of trimming is difficult to determine. These results indicate that although trimming can improve inferences in some settings, in order to consistently improve the performance of propensity score weighting, analysts should focus on the procedures leading to the generation of weights (i.e., proper specification of the propensity score model) rather than relying on ad-hoc methods such as weight trimming.},
    number = {3},
    doi = {10.1371/journal.pone.0018174}
}





@article{li2018addressing,
    author = {Li, Fan and Thomas, Laine E and Li, Fan},
    title = "{Addressing Extreme Propensity Scores via the Overlap Weights}",
    journal = {American Journal of Epidemiology},
    volume = {188},
    number = {1},
    pages = {250-257},
    year = {2018},
    month = {09},
    abstract = "{The popular inverse probability weighting method in causal inference is often hampered by extreme propensity scores, resulting in biased estimates and excessive variance. A common remedy is to trim patients with extreme scores (i.e., remove them from the weighted analysis). However, such methods are often sensitive to the choice of cutoff points and discard a large proportion of the sample. The implications for bias and the precision of the treatment effect estimate are unclear. These problems are mitigated by a newly developed method, the overlap weighting method. Overlap weights emphasize the target population with the most overlap in observed characteristics between treatments, by continuously down-weighting the units in the tails of the propensity score distribution. Here we use simulations to compare overlap weights to standard inverse probability weighting with trimming, in terms of bias, variance, and 95\% confidence interval coverage. A range of propensity score distributions are considered, including settings with substantial nonoverlap and extreme values. To facilitate practical implementation, we further provide a consistent estimator for the standard error of the treatment effect estimated using overlap weighting.}",
    issn = {0002-9262},
    doi = {10.1093/aje/kwy201},
    url = {https://doi.org/10.1093/aje/kwy201},
    eprint = {https://academic.oup.com/aje/article-pdf/188/1/250/27238730/kwy201.pdf},
}





@inproceedings{zhang2018conversations,
    title = "Conversations Gone Awry: Detecting Early Signs of Conversational Failure",
    author = "Zhang, Justine  and
      Chang, Jonathan  and
      Danescu-Niculescu-Mizil, Cristian  and
      Dixon, Lucas  and
      Hua, Yiqing  and
      Taraborelli, Dario  and
      Thain, Nithum",
    booktitle = "Proceedings of the 56th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jul,
    year = "2018",
    address = "Melbourne, Australia",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P18-1125",
    doi = "10.18653/v1/P18-1125",
    pages = "1350--1361",
    abstract = "One of the main challenges online social systems face is the prevalence of antisocial behavior, such as harassment and personal attacks. In this work, we introduce the task of predicting from the very start of a conversation whether it will get out of hand. As opposed to detecting undesirable behavior after the fact, this task aims to enable early, actionable prediction at a time when the conversation might still be salvaged. To this end, we develop a framework for capturing pragmatic devices{---}such as politeness strategies and rhetorical prompts{---}used to start a conversation, and analyze their relation to its future trajectory. Applying this framework in a controlled setting, we demonstrate the feasibility of detecting early warning signs of antisocial behavior in online discussions.",
}

@inproceedings{mirza2016catena,
    title = "{CATENA}: {CA}usal and {TE}mporal relation extraction from {NA}tural language texts",
    author = "Mirza, Paramita  and
      Tonelli, Sara",
    booktitle = "Proceedings of {COLING} 2016, the 26th International Conference on Computational Linguistics: Technical Papers",
    month = dec,
    year = "2016",
    address = "Osaka, Japan",
    publisher = "The COLING 2016 Organizing Committee",
    url = "https://www.aclweb.org/anthology/C16-1007",
    pages = "64--75",
    abstract = "We present CATENA, a sieve-based system to perform temporal and causal relation extraction and classification from English texts, exploiting the interaction between the temporal and the causal model. We evaluate the performance of each sieve, showing that the rule-based, the machine-learned and the reasoning components all contribute to achieving state-of-the-art performance on TempEval-3 and TimeBank-Dense data. Although causal relations are much sparser than temporal ones, the architecture and the selected features are mostly suitable to serve both tasks. The effects of the interaction between the temporal and the causal components, although limited, yield promising results and confirm the tight connection between the temporal and the causal dimension of texts.",
}

@misc{kingma2014adam,
    title={Adam: A Method for Stochastic Optimization},
    author={Diederik P. Kingma and Jimmy Ba},
    year={2014},
    eprint={1412.6980},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}

@article{saha2019ASM,
  title={A Social Media Study on the Effects of Psychiatric Medication Use},
  author={Koustuv Saha and Benjamin Sugar and John B Torous and Bruno D. Abrahao and Emre Kiciman and Munmun De Choudhury},
  journal={Proceedings of the ... International AAAI Conference on Weblogs and Social Media. International AAAI Conference on Weblogs and Social Media},
  year={2019},
  volume={13},
  pages={
          440-451
        }
}

@inproceedings{kiciman2018UsingLS,
  title={Using Longitudinal Social Media Analysis to Understand the Effects of Early College Alcohol Use},
  author={Emre Kiciman and Scott Counts and Melissa Gasser},
  booktitle={ICWSM},
  year={2018}
}

@article{choudhury2017language,
  title={The Language of Social Support in Social Media and Its Effect on Suicidal Ideation Risk},
  author={Munmun De Choudhury and Emre Kiciman},
  journal={Proceedings of the ... International AAAI Conference on Weblogs and Social Media. International AAAI Conference on Weblogs and Social Media},
  year={2017},
  volume={2017},
  pages={
          32-41
        }
}

@article{freedman2015reproducability,
    author = {Freedman, Leonard P. AND Cockburn, Iain M. AND Simcoe, Timothy S.},
    journal = {PLOS Biology},
    publisher = {Public Library of Science},
    title = {The Economics of Reproducibility in Preclinical Research},
    year = {2015},
    month = {06},
    volume = {13},
    url = {https://doi.org/10.1371/journal.pbio.1002165},
    pages = {1-9},
    abstract = {This Perspective provides estimates of the rate of irreproducibility of preclinical research and its direct cost implications. It goes on to outline a framework for solutions and a plan for long-term improvements in reproducibility rates.},
    number = {6},
    doi = {10.1371/journal.pbio.1002165}
}

@article{aarts2015reproducability,
author = {Aarts, Alexander and Anderson, Joanna and Anderson, Christopher and Attridge, Peter and Attwood, Angela and Axt, Jordan and Babel, Molly and Bahnik, Stepan and Baranski, Erica and Barnett-Cowan, Michael and Bartmess, Elizabeth and Beer, Jennifer and Bell, Raoul and Bentley, Heather and Beyan, Leah and Binion, Grace and Borsboom, Denny and Bosch, Annick and Bosco, Frank and Penuliar, Mike},
year = {2015},
month = {08},
pages = {},
title = {Estimating the Reproducibility of Psychological Science},
volume = {349},
journal = {Science},
doi = {10.1126/science.aac4716}
}


@article{zhang2020quantifying,
author = {Zhang, Justine and Mullainathan, Sendhil and Danescu-Niculescu-Mizil, Cristian},
title = {Quantifying the Causal Effects of Conversational Tendencies},
year = {2020},
issue_date = {October 2020},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {4},
number = {CSCW2},
url = {https://doi.org/10.1145/3415202},
doi = {10.1145/3415202},
abstract = {Understanding what leads to effective conversations can aid the design of better computer-mediated communication platforms. In particular, prior observational work has sought to identify behaviors of individuals that correlate to their conversational efficiency. However, translating such correlations to causal interpretations is a necessary step in using them in a prescriptive fashion to guide better designs and policies. In this work, we formally describe the problem of drawing causal links between conversational behaviors and outcomes. We focus on the task of determining a particular type of policy for a text-based crisis counseling platform: how best to allocate counselors based on their behavioral tendencies exhibited in their past conversations. We apply arguments derived from causal inference to underline key challenges that arise in conversational settings where randomized trials are hard to implement. Finally, we show how to circumvent these inference challenges in our particular domain, and illustrate the potential benefits of an allocation policy informed by the resulting prescriptive information.},
journal = {Proc. ACM Hum.-Comput. Interact.},
month = oct,
articleno = {131},
numpages = {24},
keywords = {counseling, conversations, causal inference}
}



@misc{gururangan2020dont,
    title={Don't Stop Pretraining: Adapt Language Models to Domains and Tasks},
    author={Suchin Gururangan and Ana Marasović and Swabha Swayamdipta and Kyle Lo and Iz Beltagy and Doug Downey and Noah A. Smith},
    year={2020},
    eprint={2004.10964},
    archivePrefix={arXiv},
    primaryClass={cs.CL}
}

@article{wang2013caliper,
    author = {Wang, Yongji AND Cai, Hongwei AND Li, Chanjuan AND Jiang, Zhiwei AND Wang, Ling AND Song, Jiugang AND Xia, Jielai},
    journal = {PLOS ONE},
    publisher = {Public Library of Science},
    title = {Optimal Caliper Width for Propensity Score Matching of Three Treatment Groups: A Monte Carlo Study},
    year = {2013},
    month = {12},
    volume = {8},
    url = {https://doi.org/10.1371/journal.pone.0081045},
    pages = {1-7},
    abstract = {Propensity score matching is a method to reduce bias in non-randomized and observational studies. Propensity score matching is mainly applied to two treatment groups rather than multiple treatment groups, because some key issues affecting its application to multiple treatment groups remain unsolved, such as the matching distance, the assessment of balance in baseline variables, and the choice of optimal caliper width. The primary objective of this study was to compare propensity score matching methods using different calipers and to choose the optimal caliper width for use with three treatment groups. The authors used caliper widths from 0.1 to 0.8 of the pooled standard deviation of the logit of the propensity score, in increments of 0.1. The balance in baseline variables was assessed by standardized difference. The matching ratio, relative bias, and mean squared error (MSE) of the estimate between groups in different propensity score-matched samples were also reported. The results of Monte Carlo simulations indicate that matching using a caliper width of 0.2 of the pooled standard deviation of the logit of the propensity score affords superior performance in the estimation of treatment effects. This study provides practical solutions for the application of propensity score matching of three treatment groups.},
    number = {12},
    doi = {10.1371/journal.pone.0081045}
}

@article{abadie2016matching,
author = {Abadie, Alberto and Imbens, Guido W.},
title = {Matching on the Estimated Propensity Score},
journal = {Econometrica},
volume = {84},
number = {2},
pages = {781-807},
keywords = {Matching estimators, propensity score matching, average treatment effects, causal inference, program evaluation},
doi = {10.3982/ECTA11293},
url = {https://onlinelibrary.wiley.com/doi/abs/10.3982/ECTA11293},
eprint = {https://onlinelibrary.wiley.com/doi/pdf/10.3982/ECTA11293},
abstract = {Propensity score matching estimators (Rosenbaum and Rubin (1983)) are widely used in evaluation research to estimate average treatment effects. In this article, we derive the large sample distribution of propensity score matching estimators. Our derivations take into account that the propensity score is itself estimated in a first step, prior to matching. We prove that first step estimation of the propensity score affects the large sample distribution of propensity score matching estimators, and derive adjustments to the large sample variances of propensity score matching estimators of the average treatment effect (ATE) and the average treatment effect on the treated (ATET). The adjustment for the ATE estimator is negative (or zero in some special cases), implying that matching on the estimated propensity score is more efficient than matching on the true propensity score in large samples. However, for the ATET estimator, the sign of the adjustment term depends on the data generating process, and ignoring the estimation error in the propensity score may lead to confidence intervals that are either too large or too small.},
year = {2016}
}



@article{hill2013common_support,
author = "Hill, Jennifer and Su, Yu-Sung",
doi = "10.1214/13-AOAS630",
fjournal = "Annals of Applied Statistics",
journal = "Ann. Appl. Stat.",
month = "09",
number = "3",
pages = "1386--1420",
publisher = "The Institute of Mathematical Statistics",
title = "Assessing lack of common support in causal inference using Bayesian nonparametrics: Implications for evaluating the effect of breastfeeding on children’s cognitive outcomes",
url = "https://doi.org/10.1214/13-AOAS630",
volume = "7",
year = "2013"
}


@article{mozer2020matching,
    title={Matching with Text Data: An Experimental Evaluation of Methods for Matching Documents and of Measuring Match Quality},
    DOI={10.1017/pan.2020.1},
    journal={Political Analysis},
    publisher={Cambridge University Press},
    author={Mozer, Reagan and Miratrix, Luke and Kaufman, Aaron Russell and Jason Anastasopoulos, L.},
    year={2020},
    pages={1–24}}

@misc{pham2017deep,
    title={A Deep Causal Inference Approach to Measuring the Effects of Forming Group Loans in Online Non-profit Microfinance Platform},
    author={Thai T. Pham and Yuanyuan Shen},
    year={2017},
    eprint={1706.02795},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@misc{sridhar2018estimating,
  title={Estimating Causal Effects of Exercise from Mood Logging Data},
  author={Dhanya Sridhar and Aaron Springer and Victoria Hollis and Steve Whittaker and Lise Getoor},
  year={2018}
}

@inproceedings{falavarjani2017estimating,
  title={Estimating the Effect Of Exercising On Users’ Online Behavior},
  author={Seyed Amin Mirlohi Falavarjani and Hawre Hosseini and Zeinab Noorian and Ebrahim Bagheri},
  booktitle={AAAI 2017},
  year={2017}
}

@article{mani2000discovery,
  title={Causal discovery from medical textual data},
  author={Subramani Mani and Gregory F. Cooper},
  journal={Proceedings. AMIA Symposium},
  year={2000},
  pages={
          542-6
        }
}

@inproceedings{fong2016discovery,
    title = "Discovery of Treatments from Text Corpora",
    author = "Fong, Christian  and
      Grimmer, Justin",
    booktitle = "Proceedings of the 54th Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = aug,
    year = "2016",
    address = "Berlin, Germany",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P16-1151",
    doi = "10.18653/v1/P16-1151",
    pages = "1600--1609",
}

@inproceedings{tan2014effect,
    title = "The effect of wording on message propagation: Topic- and author-controlled natural experiments on Twitter",
    author = "Tan, Chenhao  and
      Lee, Lillian  and
      Pang, Bo",
    booktitle = "Proceedings of the 52nd Annual Meeting of the Association for Computational Linguistics (Volume 1: Long Papers)",
    month = jun,
    year = "2014",
    address = "Baltimore, Maryland",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P14-1017",
    doi = "10.3115/v1/P14-1017",
    pages = "175--185",
}

@misc{eckles2017bias,
    title={Bias and high-dimensional adjustment in observational studies of peer effects},
    author={Dean Eckles and Eytan Bakshy},
    year={2017},
    eprint={1706.04692},
    archivePrefix={arXiv},
    primaryClass={stat.ME}
}

@article{dorie2019acic,
author = "Dorie, Vincent and Hill, Jennifer and Shalit, Uri and Scott, Marc and Cervone, Dan",
doi = "10.1214/18-STS667",
fjournal = "Statistical Science",
journal = "Statist. Sci.",
month = "02",
number = "1",
pages = "43--68",
publisher = "The Institute of Mathematical Statistics",
title = "Automated versus Do-It-Yourself Methods for Causal Inference: Lessons Learned from a Data Analysis Competition",
url = "https://doi.org/10.1214/18-STS667",
volume = "34",
year = "2019"
}


@article{jensen2019comment,
author = "Jensen, David",
doi = "10.1214/18-STS690",
fjournal = "Statistical Science",
journal = "Statist. Sci.",
month = "02",
number = "1",
pages = "77--81",
publisher = "The Institute of Mathematical Statistics",
title = "Comment: Strengthening Empirical Evaluation of Causal Inference Methods",
url = "https://doi.org/10.1214/18-STS690",
volume = "34",
year = "2019"
}


@incollection{gentzel2019evaluating,
title = {The Case for Evaluating Causal Models Using Interventional Measures and Empirical Data},
author = {Gentzel, Amanda and Garant, Dan and Jensen, David},
booktitle = {Advances in Neural Information Processing Systems 32},
editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d`Alch\'{e}-Buc and E. Fox and R. Garnett},
pages = {11722--11732},
year = {2019},
publisher = {Curran Associates, Inc.},
url = {http://papers.nips.cc/paper/9345-the-case-for-evaluating-causal-models-using-interventional-measures-and-empirical-data.pdf}
}


@book{pearl2009causality,
    place={Cambridge},
    title={Causality},
    DOI={10.1017/CBO9780511803161},
    publisher={Cambridge University Press},
    author={Pearl, Judea},
    year={2009}
}







@article{brier1950score,
author = {Brier, Glenn W.},
title = {VERIFICATION OF FORECASTS EXPRESSED IN TERMS OF PROBABILITY},
journal = {Monthly Weather Review},
volume = {78},
number = {1},
pages = {1-3},
year = {1950},
doi = {10.1175/1520-0493(1950)078<0001:VOFEIT>2.0.CO;2},

URL = { 
        https://doi.org/10.1175/1520-0493(1950)078<0001:VOFEIT>2.0.CO;2
    
},
eprint = { 
        https://doi.org/10.1175/1520-0493(1950)078<0001:VOFEIT>2.0.CO;2
    
}
,
    abstract = { Abstract No Abstract Available. }
}




@inproceedings{keith2020review,
    title = "Text and Causal Inference: A Review of Using Text to Remove Confounding from Causal Estimates",
    author={Katherine A. Keith and David Jensen and Brendan O'Connor},
    booktitle = "Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2020",
    address = "Seattle, WA",
    publisher = "Association for Computational Linguistics",
    url = "https://arxiv.org/abs/2005.00649",
    abstract = "Many applications of computational social science aim to infer causal conclusions from non-experimental data. Such observational data often contains confounders, variables that influence both potential causes and potential effects. Unmeasured or latent confounders can bias causal estimates, and this has motivated interest in measuring potential confounders from observed text. For example, an individual's entire history of social media posts or the content of a news article could provide a rich measurement of multiple confounders. Yet, methods and applications for this problem are scattered across different communities and evaluation practices are inconsistent. This review is the first to gather and categorize these examples and provide a guide to data-processing and evaluation decisions. Despite increased attention on adjusting for confounding using text, there are still many open problems, which we highlight in this paper.",
}



@Article{hajek1970,
author="H{\'a}jek, J.",
title="A characterization of limiting distributions of regular estimates",
journal="Zeitschrift f{\"u}r Wahrscheinlichkeitstheorie und Verwandte Gebiete",
year="1970",
abstract="We consider a sequence of estimates in a sequence of general estimation problems with a k-dimensional parameter. Under certain very general conditions we prove that the limiting distribution of the estimates, if properly normed, is a convolution of a certain normal distribution, which depends only of the underlying distributions, and of a further distribution, which depends on the choice of the estimate. As corollaries we obtain inequalities for asymptotic variances and for asymptotic probabilities of certain sets, generalizing so some results of J. Wolfowitz (1965), S. Kaufman (1966), L. Schmetterer (1966) and G. G. Roussas (1968).",
issn="1432-2064",
doi="",
url=""
}



@article{Blei2003LatentDA,
  title={Latent Dirichlet Allocation},
  author={D.M. Blei and A.Y. Ng and M. I. Jordan},
  journal={J. Mach. Learn. Res.},
  year={2003},
  volume={3},
  pages={993-1022}
}

@article{klein2019pathways,
    author = {Klein, C. AND Clutton, P. AND Dunn, A.G.},
    journal = {PLOS ONE},
    publisher = {Public Library of Science},
    title = {Pathways to conspiracy: The social and linguistic precursors of involvement in Reddit’s conspiracy theory forum},
    year = {2019},
    o_month = {11},
    o_volume = {14},
    url = {},
    pages = {},
    abstract = {Many individuals who engage with conspiracy theories come to do so through a combination of individual and social factors. The interaction between these factors is challenging to study using traditional experimental designs. Reddit.com is a large connected set of online discussion forums, including one (r/conspiracy) devoted to wide-ranging discussion of conspiracy theories. The availability of large datasets of user comments from Reddit give a unique opportunity to observe human behavior in social spaces and at scale. Using a retrospective case control study design, we analyzed how Reddit users who would go on to engage with a conspiracy-related forum differed from other users in the language they use, differences in the social environments where they posted, and potential interactions between the two factors. Together, the analyses provide evidence for self-selection into communities with a shared set of interests which can feed into a conspiratorial world-view, and that these differences are detectable relative to controls even before users begin to post in r/conspiracy. We also suggest that survey-based and experimental studies may benefit from differentiating between passive private endorsement by individuals and active engagement with conspiracy theories in social spaces.},
    number = {11},
    doi = {}
}

@inproceedings{bhattacharya2016information,
author = {Bhattacharya, P. and Mehrotra, R.},
title = {The Information Network: Exploiting Causal Dependencies in Online Information Seeking},
year = {2016},
isbn = {9781450337519},
publisher = {},
address = {},
o_url = {},
o_doi = {},
booktitle = {Proceedings of the 2016 ACM on Conference on Human Information Interaction and Retrieval},
pages = {},
numpages = {10},
keywords = {information seeking, granger causality, recommendations},
location = {Carrboro, North Carolina, USA},
series = {CHIIR ’16}
}
  


@article{chandrasekharan2017ban,
author = {Chandrasekharan, Eshwar and Pavalanathan, Umashanthi and Srinivasan, Anirudh and Glynn, Adam and Eisenstein, Jacob and Gilbert, Eric},
title = {You Can’t Stay Here: The Efficacy of Reddit’s 2015 Ban Examined Through Hate Speech},
year = {2017},
issue_date = {November 2017},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {1},
number = {CSCW},
url = {https://doi.org/10.1145/3134666},
doi = {10.1145/3134666},
journal = {Proc. ACM Hum.-Comput. Interact.},
month = dec,
articleno = {31},
numpages = {22},
keywords = {online communities, moderation, hate speech, causal inference, banning}
}
  

  


@misc{hahn2019atlantic,
    title={Atlantic Causal Inference Conference (ACIC) Data Analysis Challenge 2017},
    author={P.R. Hahn and V. Dorie and J.S. Murray},
    year={2019},
    eprint={1905.09515},
    archivePrefix={arXiv},
    primaryClass={stat.ME}
}

@article{pearl1995causal,
 ISSN = {00063444},
 URL = {},
 abstract = {The primary aim of this paper is to show how graphical models can be used as a mathematical language for integrating statistical and subject-matter information. In particular, the paper develops a principled, nonparametric framework for causal inference, in which diagrams are queried to determine if the assumptions available are sufficient for identifying causal effects from nonexperimental data. If so the diagrams can be queried to produce mathematical expressions for causal effects in terms of observed distributions; otherwise, the diagrams can be queried to suggest additional observations or auxiliary experiments from which the desired inferences can be obtained.},
 author = {Judea Pearl},
 journal = {Biometrika},
 number = {4},
 pages = {},
 publisher = {[Oxford University Press, Biometrika Trust]},
 title = {Causal Diagrams for Empirical Research},
 volume = {82},
 year = {1995}
}


@inproceedings{olteanu2017distilling,
author = {Olteanu, Alexandra and Varol, Onur and Kiciman, Emre},
title = {Distilling the Outcomes of Personal Experiences: A Propensity-Scored Analysis of Social Media},
year = {2017},
isbn = {9781450343350},
publisher = {},
address = {},
o_url = {},
o_doi = {},
booktitle = {Proceedings of the 2017 ACM Conference on Computer Supported Cooperative Work and Social Computing},
pages = {},
numpages = {17},
keywords = {information extraction, social media, experience outcomes},
location = {Portland, Oregon, USA},
series = {CSCW ’17}
}

@misc{arbour2019permutation,
    title={Permutation Weighting},
    author={David Arbour and Drew Dimmery},
    year={2019},
    eprint={1901.01230},
    archivePrefix={arXiv},
    primaryClass={stat.ME}
}

@misc{baumgartner2020pushshift,
    title={The Pushshift Reddit Dataset},
    author={Jason Baumgartner and Savvas Zannettou and Brian Keegan and Megan Squire and Jeremy Blackburn},
    year={2020},
    eprint={2001.08435},
    archivePrefix={arXiv},
    primaryClass={cs.SI}
}

@inproceedings{paul2017feature,
  title={Feature selection as causal inference: Experiments with text classification},
  author={Paul, Michael J},
  booktitle={Proceedings of the 21st Conference on Computational Natural Language Learning (CoNLL 2017)},
  pages={163--172},
  year={2017}
}

@misc{roberts2018adjusting,
  title={Adjusting for confounding with text matching},
  author={Roberts, Margaret E and Stewart, Brandon M and Nielsen, Richard A},
  booktitle={American Journal of Political Science (forthcoming)},
  year={2020}
}

@inproceedings{d2019multi,
  title={On multi-cause approaches to causal inference with unobserved counfounding: Two cautionary failure cases and a promising alternative},
  author={D’Amour, Alexander},
  booktitle={AISTATS},
  pages={},
  year={2019}
}

@article{wang2019blessings,
  title={The blessings of multiple causes},
  author={Wang, Yixin and Blei, David M},
  journal={Journal of the American Statistical Association},
  number={1},
  pages={},
  year={2019},
  publisher={Taylor \& Francis}
}

@article{ranganath2018multiple,
  title={Multiple causal inference with latent confounding},
  author={Ranganath, Rajesh and Perotte, Adler},
  journal={arXiv:1805.08273},
  year={2018}
}


@article{peters2018deep,
  title={Deep contextualized word representations},
  author={Peters, Matthew E and Neumann, Mark and Iyyer, Mohit and Gardner, Matt and Clark, Christopher and Lee, Kenton and Zettlemoyer, Luke},
  journal={arXiv:1802.05365},
  year={2018}
}

@inproceedings{yao2019estimation,
  title={On the estimation of treatment effect with text covariates},
  author={Yao, Liuyi and Li, Sheng and Li, Yaliang and Xue, Hongfei and Gao, Jing and Zhang, Aidong},
  booktitle={IJCAI},
  pages={},
  year={2019},
}

@article{mayer2019doubly,
  title={Doubly robust treatment effect estimation with missing attributes},
  author={Mayer, Imke and Wager, Stefan and Gauss, Tobias and Moyer, Jean-Denis and Josse, Julie},
  journal={arXiv:1910.10624},
  year={2019}
}

@inproceedings{louizos2017causal,
  title={Causal effect inference with deep latent-variable models},
  author={Louizos, Christos and Shalit, Uri and Mooij, Joris M and Sontag, David and Zemel, Richard and Welling, Max},
  booktitle={NeurIPS},
  pages={},
  year={2017}
}

@article{kuroki2014measurement,
  title={Measurement bias and effect restoration in causal inference},
  author={Kuroki, Manabu and Pearl, Judea},
  journal={Biometrika},
  volume={101},
  number={2},
  pages={},
  year={2014},
}

@inproceedings{kallus2018causal,
  title={Causal inference with noisy and missing covariates via matrix factorization},
  author={Kallus, Nathan and Mao, Xiaojie and Udell, Madeleine},
  booktitle={NeurIPS},
  pages={},
  year={2018}
}

@article{kuroki1999identifiability,
  title={Identifiability criteria for causal effects of joint interventions},
  author={Kuroki, Manabu and Miyakawa, Masami},
  journal={Journal of the Japan Statistical Society},
  volume={29},
  number={2},
  o_pages={105--117},
  year={1999},
}

@inproceedings{pearl2012measurement,
author = {Pearl, Judea},
title = {On Measurement Bias in Causal Inference},
year = {2010},
isbn = {9780974903965},
publisher = {AUAI Press},
address = {Arlington, Virginia, USA},
booktitle = {Proceedings of the Twenty-Sixth Conference on Uncertainty in Artificial Intelligence},
pages = {425–432},
numpages = {8},
location = {Catalina Island, CA},
series = {UAI’10}
}



@article{miao2018identifying,
  title={Identifying causal effects with proxy variables of an unmeasured confounder},
  author={Miao, Wang and Geng, Zhi and Tchetgen Tchetgen, Eric J},
  journal={Biometrika},
  volume={105},
  number={4},
  pages={},
  year={2018},
  publisher={Oxford University Press}
}



@article{yang2018asymptotic,
    author = {Yang, S and Ding, P},
    title = "{Asymptotic inference of causal effects with observational studies trimmed by the estimated propensity scores}",
    journal = {Biometrika},
    volume = {105},
    number = {2},
    pages = {487-493},
    year = {2018},
    month = {03},
    abstract = "{Causal inference with observational studies often relies on the assumptions of unconfoundedness and overlap of covariate distributions in different treatment groups. The overlap assumption is violated when some units have propensity scores close to \\$0\\$ or \\$1\\$, so both practical and theoretical researchers suggest dropping units with extreme estimated propensity scores. However, existing trimming methods often do not incorporate the uncertainty in this design stage and restrict inference to only the trimmed sample, due to the nonsmoothness of the trimming. We propose a smooth weighting, which approximates sample trimming and has better asymptotic properties. An advantage of our estimator is its asymptotic linearity, which ensures that the bootstrap can be used to make inference for the target population, incorporating uncertainty arising from both design and analysis stages. We extend the theory to the average treatment effect on the treated, suggesting trimming samples with estimated propensity scores close to \\$1\\$.}",
    issn = {0006-3444},
    doi = {10.1093/biomet/asy008},
    url = {https://doi.org/10.1093/biomet/asy008},
    eprint = {https://academic.oup.com/biomet/article-pdf/105/2/487/24821001/asy008.pdf},
}

 

@inproceedings{yao2018representation,
  title={Representation learning for treatment effect estimation from observational data},
  author={Yao, Liuyi and Li, Sheng and Li, Yaliang and Huai, Mengdi and Gao, Jing and Zhang, Aidong},
  booktitle={NeurIPS},
  pages={},
  year={2018}
}


@inproceedings{johansson2016learning,
  title={Learning representations for counterfactual inference},
  author={Johansson, Fredrik and Shalit, Uri and Sontag, David},
  booktitle={ICML},
  o_pages={},
  year={2016}
}

 

@article{Hazlehurst2009DetectingPV,
  title={Detecting possible vaccine adverse events in clinical notes of the electronic medical record.},
  author={Brian Hazlehurst and Allison L Naleway and John P. Mullooly},
  journal={Vaccine},
  year={2009},
  volume={27 14},
  pages={
          2077-83
        }
}

@inproceedings{kale2015causal,
  title={Causal phenotype discovery via deep networks},
  author={Kale, David C and Che, Zhengping and Bahadori, Mohammad Taha and Li, Wenzhe and Liu, Yan and Wetzel, Randall},
  booktitle={AMIA},
  volume={},
  pages={},
  year={2015},
  o_organization={American Medical Informatics Association}
}

 

@article{spertus2018bayesian,
  title={Bayesian propensity scores for high-dimensional causal inference: A comparison of drug-eluting to bare-metal coronary stents},
  author={Spertus, Jacob V and Normand, Sharon-Lise T},
  journal={Biometrical Journal},
  volume={60},
  number={4},
  pages={721--733},
  year={2018},
  publisher={Wiley Online Library}
}

 

@article{qin2019using,
  title={Using a monotone single-index model to stabilize the propensity score in missing data problems and causal inference},
  author={Qin, Jing and Yu, Tao and Li, Pengfei and Liu, Hao and Chen, Baojiang},
  journal={Statistics in medicine},
  volume={38},
  number={8},
  pages={1442--1458},
  year={2019},
  publisher={Wiley Online Library}
}

 


 @misc{kyriakakis2019transfer,
    title={Transfer Learning for Causal Sentence Detection},
    author={Manolis Kyriakakis and Ion Androutsopoulos and Joan Ginés i Ametllé and Artur Saudabayev},
    year={2019},
    eprint={1906.07544},
    archivePrefix={arXiv},
    primaryClass={cs.CL}
}

@inproceedings{rehman2016using,
  title={Using propensity score matching to understand the relationship between online health information sources and vaccination sentiment},
  author={Rehman, N and Liu, Jason and Chunara, Rumi},
  booktitle={Proceedings of Association for the Advancement of Artificial Intelligence Spring Symposia},
  pages={23--25},
  year={2016}
}

 

@article{afzal2019generating,
  title={Generating and evaluating a propensity model using textual features from electronic medical records},
  author={Afzal, Zubair and Masclee, Gwen MC and Sturkenboom, Miriam CJM and Kors, Jan A and Schuemie, Martijn J},
  journal={PloS one},
  volume={14},
  number={3},
  pages={e0212999},
  year={2019},
  publisher={Public Library of Science}
}

 

@inproceedings{ruchansky2017csi,
  title={Csi: A hybrid deep model for fake news detection},
  author={Ruchansky, Natali and Seo, Sungyong and Liu, Yan},
  booktitle={Proceedings of the ACM Conference on Information and Knowledge Management},
  pages={797--806},
  year={2017},
  organization={ACM}
}

 

@inproceedings{singh2016cyberbullying,
  title={Cyberbullying detection using probabilistic socio-textual information fusion},
  author={Singh, Vivek K and Huang, Qianjia and Atrey, Pradeep K},
  booktitle={Proceedings of the 2016 IEEE/ACM International Conference on Advances in Social Networks Analysis and Mining},
  pages={884--887},
  year={2016},
  organization={IEEE Press}
}

@inproceedings{dechoudhury2016mental_chi,
 author = {De Choudhury, Munmun and Kiciman, Emre and Dredze, Mark and Coppersmith, Glen and Kumar, Mrinal},
 title = {Discovering Shifts to Suicidal Ideation from Mental Health Content in Social Media},
 year = {2016},
 isbn = {9781450333627},
 publisher = {},
 address = {},
 url = {},
 doi = {},
 booktitle = {Proceedings of the 2016 CHI Conference on Human Factors in Computing Systems},
 pages = {},
 numpages = {},
 keywords = {reddit, suicidal ideation, mental health, social media},
 location = {San Jose, California, USA},
 series = {CHI ’16}
}

@book{rosenbaum_2010,
  place={New York},
  title={Design of Observational Studies},
  publisher={Springer}, author={Rosenbaum, Paul R.},
  year={2010}
}

@article{veitch2019embeddings,
  author    = {Victor Veitch and
               Dhanya Sridhar and
               David M. Blei},
  title     = {Using Text Embeddings for Causal Inference},
  journal   = {CoRR},
  volume    = {abs/1905.12741},
  year      = {2019},
  o_url       = {http://arxiv.org/abs/1905.12741},
  archivePrefix = {arXiv},
  eprint    = {1905.12741},
  timestamp = {Mon, 03 Jun 2019 13:42:33 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1905-12741},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{wood_doughty2018challenges,
    title = "Challenges of Using Text Classifiers for Causal Inference",
    author = "Wood-Doughty, Zach  and
      Shpitser, Ilya  and
      Dredze, Mark",
    booktitle = "Proceedings of the 2018 Conference on Empirical Methods in Natural Language Processing",
    month = oct # "-" # nov,
    year = "2018",
    address = "Brussels, Belgium",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/D18-1488",
    doi = "10.18653/v1/D18-1488",
    pages = "4586--4598",
    abstract = "Causal understanding is essential for many kinds of decision-making, but causal inference from observational data has typically only been applied to structured, low-dimensional datasets. While text classifiers produce low-dimensional outputs, their use in causal inference has not previously been studied. To facilitate causal analyses based on language data, we consider the role that text classifiers can play in causal inference through established modeling mechanisms from the causality literature on missing data and measurement error. We demonstrate how to conduct causal analyses using text classifiers on simulated and Yelp data, and discuss the opportunities and challenges of future work that uses text data in causal inference.",
}

@misc{egami2018make,
    title={How to Make Causal Inferences Using Texts},
    author={Naoki Egami and Christian J. Fong and Justin Grimmer and Margaret E. Roberts and Brandon M. Stewart},
    year={2018},
    eprint={1802.02163},
    archivePrefix={arXiv},
    primaryClass={stat.ML}
}

@article{bareinboim2016causal,
  title={Causal inference and the data-fusion problem},
  author={Bareinboim, Elias and Pearl, Judea},
  journal={Proceedings of the National Academy of Sciences},
  volume={113},
  number={27},
  pages={7345--7352},
  year={2016},
  publisher={National Acad Sciences}
}
@article{glynn2010introduction,
  title={An introduction to the augmented inverse propensity weighted estimator},
  author={Glynn, Adam N and Quinn, Kevin M},
  journal={Political analysis},
  volume={18},
  number={1},
  pages={36--56},
  year={2010},
  publisher={Cambridge University Press}
}

@inproceedings{zhang-etal-2019-hibert,
    title = "{HIBERT}: Document Level Pre-training of Hierarchical Bidirectional Transformers for Document Summarization",
    author = "Zhang, Xingxing  and
      Wei, Furu  and
      Zhou, Ming",
    booktitle = "ACL",
    month = jul,
    year = "2019",
    address = "",
    publisher = "",
    o_url = "",
    doi = "",
    pages = "",
}

@inproceedings{devlin-etal-2019-bert,
    title = "{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding",
    author = "Devlin, Jacob  and
      Chang, Ming-Wei  and
      Lee, Kenton  and
      Toutanova, Kristina",
    booktitle = "NAACL",
    month = jun,
    year = "2019",
    address = "",
    publisher = "",
    o_url = "",
    o_doi = "",
    o_pages = "4171--4186",

}

@article{pourhoseingholi2012control,
  title={How to control confounding effects by statistical analysis},
  author={Pourhoseingholi, Mohamad Amin and Baghestani, Ahmad Reza and Vahedi, Mohsen},
  journal={Gastroenterology and Hepatology from bed to bench},
  volume={5},
  number={2},
  pages={79},
  year={2012},
  publisher={Shahid Beheshti University of Medical Sciences}
}
